Early Planet Formation in Embedded Disks (eDisk). VII. Keplerian Disk, Disk Substructure, and Accretion Streamers in the Class 0 Protostar IRAS 16544-1604 in CB 68

We present observations of the Class 0 protostar IRAS 16544-1604 in CB 68 from the ''Early Planet Formation in Embedded Disks (eDisk)'' ALMA Large program. The ALMA observations target continuum and lines at 1.3-mm with an angular resolution of $\sim$5 au. The continuum image reveals a dusty protostellar disk with a radius of $\sim$30 au seen close to edge-on, and asymmetric structures both along the major and minor axes. While the asymmetry along the minor axis can be interpreted as the effect of the dust flaring, the asymmetry along the major axis comes from a real non-axisymmetric structure. The C$^{18}$O image cubes clearly show the gas in the disk that follows a Keplerian rotation pattern around a $\sim$0.14 $M_{\odot}$ central protostar. Furthermore, there are $\sim$1500 au-scale streamer-like features of gas connecting from North-East, North-North-West, and North-West to the disk, as well as the bending outflow as seen in the $^{12}$CO (2-1) emission. At the apparent landing point of NE streamer, there are SO (6$_5$-5$_4$) and SiO (5-4) emission detected. The spatial and velocity structure of NE streamer can be interpreted as a free-falling gas with a conserved specific angular momentum, and the detection of the SO and SiO emission at the tip of the streamer implies presence of accretion shocks. Our eDisk observations have unveiled that the Class 0 protostar in CB 68 has a Keplerian rotating disk with flaring and non-axisymmetric structure associated with accretion streamers and outflows.

==> CB68_molecular_line.tex <==

\begin{deluxetable*}{ccccccccc}
%\centering
\caption{Observed Molecular Lines}
\label{table:CB68_molecular_line}
\tablehead{
    \colhead{Molecule} & \colhead{Transition} & \colhead{Frequency} & \colhead{$E_u$$^{a,b}$} & \colhead{$A^{b,c}$} & \colhead{$n_{crit}$$^{b,d}$} & \colhead{Beam Size} & \colhead{$\Delta$$v^e$} & \colhead{rms}\\
    \colhead{} &\colhead{} &\colhead{(GHz)} &\colhead{(K)} &\colhead{(s$^{-1}$)} &\colhead{(cm$^{-3}$)} &\colhead{} & \colhead{(km s$^{-1}$)} & \colhead{(mJy beam$^{-1}$)}
}
\startdata
    $^{12}$CO & 2--1 & 230.538 & 16.60 & 6.910 $\times$ 10$^{-7}$ & 1.1 $\times$ 10$^4$ & 0$\farcs$24 $\times$ 0$\farcs$18 (P.A.=79$\degr$) & 0.635 & 1.2\\
    C$^{18}$O & 2--1 & 219.560 & 15.81 & 6.011 $\times$ 10$^{-7}$ & 9.3 $\times$ 10$^3$ & 0$\farcs$27 $\times$ 0$\farcs$20 (P.A.=77$\degr$)& 0.167 & 1.9\\
    $^{13}$CO & 2--1 & 220.399 & 15.87 & 6.038 $\times$ 10$^{-7}$ & 9.4 $\times$ 10$^3$ & 0$\farcs$24 $\times$ 0$\farcs$18 (P.A.=81$\degr$) & 0.167 & 2.5\\
    SO & 6$_5$--5$_4$ & 219.995 & 35.0 & 1.335 $\times$ 10$^{-4}$ & 2.3 $\times$ 10$^6$ & 0$\farcs$27 $\times$ 0$\farcs$20 (P.A.=77$\degr$) & 0.167 & 2.4\\
    %not (high T) ver.
    SiO & 5--4 & 219.949 & 31.26 & 5.197 $\times$ 10$^{-4}$ & 2.4 $\times$ 10$^6$ & 0$\farcs$25 $\times$ 0$\farcs$19 (P.A.=79$\degr$) & 1.34 & 0.7\\
    %hcn.dat (265.88643390 GHz)
    DCN$^f$ & 3--2 & 217.239 & 20.85 & 4.57 $\times$ 10$^{-4}$ & 3.7 $\times$ 10$^7$ & 0$\farcs$25  $\times$ 0$\farcs$19 (P.A.=79$\degr$) & 1.34 & 0.7\\
    %e-CH3OH
    CH$_3$OH & 4$_2$--3$_1$ & 218.440 & 45.5 & 4.686 $\times$ 10$^{-5}$ & 2.0 $\times$ 10$^7$ & 0$\farcs$25  $\times$ 0$\farcs$19 (P.A.=79$\degr$) & 1.34 & 0.6\\
    %p-C3H2
    $c$-C$_3$H$_2$ & 6$_{0,6}$--5$_{1,5}$ & 217.822 & 38.61 & 5.393 $\times$ 10$^{-4}$ & 4.5 $\times$ 10$^7$ & 0$\farcs$25 $\times$ 0$\farcs$19 (P.A.=79$\degr$) & 1.34 & 0.7\\
            %o-C3H2
    & 5$_{1,4}$--4$_{2,3}$ & 217.940 & 35.42 & 4.023 $\times$ 10$^{-4}$ & 4.8 $\times$ 10$^7$ & 0$\farcs$25 $\times$ 0$\farcs$19 (P.A.=79$\degr$) & 1.34 & 0.6\\
             %p-C3H2
    & 5$_{2,4}$--4$_{1,3}$ & 218.160 & 35.42 & 4.039 $\times$ 10$^{-4}$ & 4.8 $\times$ 10$^7$ & 0$\farcs$25  $\times$ 0$\farcs$19 (P.A.=79$\degr$) & 1.34 & 0.6\\
    %ph2co-h2.dat         
    H$_2$CO & 3$_{0,3}$--2$_{0,2}$ & 218.222 & 21.0 & 2.818 $\times$ 10$^{-4}$ & 2.6 $\times$ 10$^6$ & 0$\farcs$25  $\times$ 0$\farcs$19 (P.A.=79$\degr$) & 1.34 & 0.6\\
          %ph2co-h2.dat  
    & 3$_{2,2}$--2$_{2,1}$ & 218.476 & 68.1 & 1.571 $\times$ 10$^{-4}$ & 3.0 $\times$ 10$^6$ & 0$\farcs$35  $\times$ 0$\farcs$26 (P.A.=78$\degr$) & 1.34 & 0.6\\
          %ph2co-h2.dat  
    & 3$_{2,1}$--2$_{2,0}$ & 218.760 & 68.1 & 1.577 $\times$ 10$^{-4}$ & 3.4 $\times$ 10$^6$& 0$\farcs$26  $\times$ 0$\farcs$20 (P.A.=77$\degr$) & 0.167 & 1.8\\
\enddata 
\tablecomments{$^a$Upper state energy of the line.\\
$^b$From the LAMDA database \citep{Schoier2005}.\\
$^c$Einstein $A$ coefficient.\\
$^d$Critical density at $T_K$ =20 K, except for that of the SO and c-C$_3$H$_2$ lines which adopt 60 K and 30 K, respectively.\\ 
\hspace{4pt}Calculated from the Einstein $A$- and $C$-coefficients from the LAMDA database.\\
$^e$Velocity resolution.\\
$^f$$E_u$ and $A$ values are from the CDMS database \citep{2001Muller,2005Muller,2016Endres}.\\
\hspace{4pt}The $C$-coefficient of the HCN line is adopted.
}
\end{deluxetable*}


==> CB68_observations.tex <==
\begin{deluxetable*}{lcccc}
\tablewidth{\textwidth}
\caption{Observational Parameters}
\label{table:obs}
\tablehead{
\colhead{Project code} & \multicolumn{3}{c}{2019.1.00261.L} & \colhead{2019.A.00034.S}
}
\startdata
Observing date & 24 Aug. 2021 & 04 Oct. 2021 & 05 Oct. 2021 & 14 Jun. 2022\\
Number of antennas & 50 & 45 & 46 & 42\\
Configuration & \multicolumn{3}{c}{C-8} & C-4\\
Phase center & \multicolumn{4}{c}{( 16$^h$57$^m$19$\fs$64, $-$16$^d$09$^m$23$\fs$9) (ICRS)}\\ 
Synthesized beam (continuum, robust$=$0.0) & \multicolumn{4}{c}{0$\farcs$036 $\times$ 0$\farcs$027 (P.A.$=$69$\degr$)}\\%restoring beam
Conversion factor (continuum, robust$=$0.0) & \multicolumn{4}{c}{1 Jy beam$^{-1}$$=$6036 $\rm{K}$}\\
Noise level (continuum, robust$=$0.0) & \multicolumn{4}{c}{21 $\mu$Jy beam$^{-1}$$=$5 $\rm{K}$}
\enddata
%\tablenotetext{a}{Using the Rayleigh-Jeans approximately.}
\end{deluxetable*}
